Generating Adversarial Examples with Task Oriented Multi-Objective Optimization

Deep learning models, even the-state-of-the-art ones, are highly vulnerable to adversarial examples. Adversarial training is one of the most efficient methods to improve the model's robustness. The key factor for the success of adversarial training is the capability to generate qualified and divergent adversarial examples which satisfy some objectives/goals (e.g., finding adversarial examples that maximize the model losses for simultaneously attacking multiple models). Therefore, multi-objective optimization (MOO) is a natural tool for adversarial example generation to achieve multiple objectives/goals simultaneously. However, we observe that a naive application of MOO tends to maximize all objectives/goals equally, without caring if an objective/goal has been achieved yet. This leads to useless effort to further improve the goal-achieved tasks, while putting less focus on the goal-unachieved tasks. In this paper, we propose \emph{Task Oriented MOO} to address this issue, in the context where we can explicitly define the goal achievement for a task. Our principle is to only maintain the goal-achieved tasks, while letting the optimizer spend more effort on improving the goal-unachieved tasks. We conduct comprehensive experiments for our Task Oriented MOO on various adversarial example generation schemes. The experimental results firmly demonstrate the merit of our proposed approach. Our code is available at \url{https://github.com/tuananhbui89/TAMOO}.

==> moo_checklist.tex <==




\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See the discussion in Appendix E.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{The main results and lemmas appear in the main paper while their complete proof can be found in Appendix B.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{The code will be published upon the acceptance of the paper.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See the setting detail in Appendix C.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{We set the same random seed for all experiments and did not tune this parameter.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See the setting detail in Appendix C.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited the authors of the codes and datasets that we used in our experiments.}
  \item Did you mention the license of the assets?
    \answerNA{All the assets we used are published for research purposes.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All the assets we used are published for research purposes.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{All the assets we used are published for research purposes.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> theory.tex <==
\section{New Theory}

\begin{restatable}{thm}{theorem3}\label{theorem3}
    Given $m$ tasks and Pareto optimality point $\delta_m^* = \underset{\delta}{\text{argmax}} \left[ f_i \left( \delta \right) \right]_{i=1}^m$. 
    Then given an abitrary subset from $m$ tasks, for example, without loss of generality, 
    the first $s$ tasks from $m$ tasks (i.e., $ 1 \leq s \leq m$). 
    Then the above Pareto optimality point is also the Pareto optimality point for the new set of tasks. 
    
    $\delta_s^* = \underset{\delta}{\text{argmax}} \left[ f_i \left( \delta \right) \right]_{i=1}^s$. 
    and $\delta_s^* = \delta_m^*$
\end{restatable}

\begin{restatable}{thm}{theorem4}\label{theorem4}
    When reaching the Pareto optimality point $\delta*$ at which there exist $w\in\simplex_{m}$ such
    that $\sum_{i=1}^{m}w_{i}\nabla_{\delta}f_{i}\left(\delta^{*}\right)=\bzero$. 
    Given an abitrary subset from $m$ tasks, for example, without loss of generality, 
    the first $s$ tasks from $m$ tasks (i.e., $ 1 \leq s \leq m$). 
    There is also exist $w^s \in\simplex_{s}$ such that 
    $\sum_{i=1}^{s}w_{i}^s\nabla_{\delta}f_{i}\left(\delta^{*}\right)=\bzero$
\end{restatable}
